Sequence Numbers Do Not Guarantee Loop Freedom; AODV Can Yield Routing Loops

In the area of mobile ad-hoc networks and wireless mesh networks, sequence numbers are often used in routing protocols to avoid routing loops. It is commonly stated in protocol specifications that sequence numbers are sufficient to guarantee loop freedom if they are monotonically increased over time. A classical example for the use of sequence numbers is the popular Ad hoc On-Demand Distance Vector (AODV) routing protocol. The loop freedom of AODV is not only a common belief, it has been claimed in the abstract of its RFC and at least two proofs have been proposed. AODV-based protocols such as AODVv2 (DYMO) and HWMP also claim loop freedom due to the same use of sequence numbers. In this paper we show that AODV is not a priori loop free; by this we counter the proposed proofs in the literature. In fact, loop freedom hinges on non-evident assumptions to be made when resolving ambiguities occurring in the RFC. Thus, monotonically increasing sequence numbers, by themselves, do not guarantee loop freedom.

==> fig/ex_loop_1.tex <==
%% Latex Commands%%
\newcommand{\msg}[3]{#1${}_{\!\!\;\MakeUppercase{#2}\!\!\:\shortrightarrow\!\MakeUppercase{#3}}$}
\newcommand{\msgerr}{RERR}
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(5.0,2.0){0.28}{x}
   \rput(5.0,2.091){\small$X$}
   \rput(5.0,1.8599999999999999){\tiny $1$}
\rput(5.0,2.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}
   \rput(2.6,0.0){\includegraphics[scale=0.13]{cloud.eps}}
   \cnode(0.0,0.0){0.28}{a}
   \rput(0.0,0.091){\small$A$}
   \rput(0.0,-0.14){\tiny $1$}
\rput(0.0,-0.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}
   \pnode(2.5,0.45){Cu}
   \cnode(0.0,2.0){0.28}{d}
   \rput(0.0,2.091){\small$D$}
   \rput(0.0,1.8599999999999999){\tiny $1$}
\rput(0.0,2.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}
   \pnode(1.45,0.0){Cl}
   \cnode(2.5,2.0){0.28}{s}
   \rput(2.5,2.091){\small$S$}
   \rput(2.5,1.8599999999999999){\tiny $1$}
\rput(2.5,2.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}

%%  EDGES  %%
   \ncline{a}{Cl}
   \ncline{a}{d}
   \ncline{Cu}{s}

%%  MSGS  %%

\endpspicture


==> fig/ex_loop_2.tex <==
%% Latex Commands%%
\newcommand{\msg}[3]{#1${}_{\!\!\;\MakeUppercase{#2}\!\!\:\shortrightarrow\!\MakeUppercase{#3}}$}
\newcommand{\msgerr}{RERR}
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(5.0,2.0){0.28}{x}
   \rput(5.0,2.091){\small$X$}
   \rput(5.0,1.8599999999999999){\tiny $1$}
\rput(5.0,2.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}
   \rput(2.6,0.0){\includegraphics[scale=0.13]{cloud.eps}}
   \cnode(0.0,0.0){0.28}{a}
   \rput(0.0,0.091){\small$A$}
   \rput(0.0,-0.14){\tiny $1$}
\rput(0.0,-0.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (D & 2 & \mbox{val} & 1 & D)\\
   \end{array}$}

}
   \pnode(2.5,0.45){Cu}
   \cnode(0.0,2.0){0.28}{d}
   \rput(0.0,2.091){\small$D$}
   \rput(0.0,1.8599999999999999){\tiny $2$}
\rput(0.0,2.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 1 & \mbox{val} & 1 & A)\\
   \end{array}$}

}
   \pnode(1.45,0.0){Cl}
   \cnode(2.5,2.0){0.28}{s}
   \rput(2.5,2.091){\small$S$}
   \rput(2.5,1.8599999999999999){\tiny $1$}
\rput(2.5,2.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}

%%  EDGES  %%
   \ncline{a}{Cl}
   \ncline{a}{d}
   \ncline{Cu}{s}

%%  MSGS  %%
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{<-}{d}{a}
   \aput[1pt]{:D}{\tiny \msg{RREP}{d}{a}}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{<-}{a}{d}
   \aput[1pt]{:U}{\tiny \msg{RREQ}{d}{a}}

\endpspicture


==> fig/ex_loop_3.tex <==
%% Latex Commands%%
\newcommand{\msg}[3]{#1${}_{\!\!\;\MakeUppercase{#2}\!\!\:\shortrightarrow\!\MakeUppercase{#3}}$}
\newcommand{\msgerr}{RERR}
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(5.0,2.0){0.28}{x}
   \rput(5.0,2.091){\small$X$}
   \rput(5.0,1.8599999999999999){\tiny $1$}
\rput(5.0,2.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}
   \rput(2.6,0.0){\includegraphics[scale=0.13]{cloud.eps}}
   \cnode(0.0,0.0){0.28}{a}
   \rput(0.0,0.091){\small$A$}
   \rput(0.0,-0.14){\tiny $1$}
\rput(0.0,-0.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (D & 2 & \mbox{val} & 1 & D)\\
   \end{array}$}

}
   \pnode(2.5,0.45){Cu}
   \cnode(0.0,2.0){0.28}{d}
   \rput(0.0,2.091){\small$D$}
   \rput(0.0,1.8599999999999999){\tiny $2$}
\rput(0.0,2.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 1 & \mbox{val} & 1 & A)\\
   \end{array}$}

}
   \pnode(1.45,0.0){Cl}
   \cnode(2.5,2.0){0.28}{s}
   \rput(2.5,2.091){\small$S$}
   \rput(2.5,1.8599999999999999){\tiny $2$}
\rput(2.5,2.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}

%%  EDGES  %%
   \ncline{a}{Cl}
   \ncline{a}{d}
   \ncline{Cu}{s}

%%  MSGS  %%
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{<->}{s}{Cu}
   \aput[1pt]{:D}{\tiny \msg{RREQ}{s}{d}}

\endpspicture


==> fig/ex_loop_4.tex <==
%% Latex Commands%%
\newcommand{\msg}[3]{#1${}_{\!\!\;\MakeUppercase{#2}\!\!\:\shortrightarrow\!\MakeUppercase{#3}}$}
\newcommand{\msgerr}{RERR}
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(5.0,2.0){0.28}{x}
   \rput(5.0,2.091){\small$X$}
   \rput(5.0,1.8599999999999999){\tiny $1$}
\rput(5.0,2.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}
   \rput(2.6,0.0){\includegraphics[scale=0.13]{cloud.eps}}
   \cnode(0.0,0.0){0.28}{a}
   \rput(0.0,0.091){\small$A$}
   \rput(0.0,-0.14){\tiny $1$}
\rput(0.0,-0.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (D & 2 & \mbox{val} & 1 & D)\\
       (S & 3 & \mbox{val} & 2 & D)\\
   \end{array}$}

}
   \pnode(2.5,0.45){Cu}
   \cnode(0.0,2.0){0.28}{d}
   \rput(0.0,2.091){\small$D$}
   \rput(0.0,1.8599999999999999){\tiny $2$}
\rput(0.0,2.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 1 & \mbox{val} & 1 & A)\\
       (S & 3 & \mbox{val} & 1 & S)\\
   \end{array}$}

}
   \pnode(1.45,0.0){Cl}
   \cnode(2.5,2.0){0.28}{s}
   \rput(2.5,2.091){\small$S$}
   \rput(2.5,1.8599999999999999){\tiny $3$}
\rput(2.5,2.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (D & 0 & \mbox{val} & 1 & D)\\
   \end{array}$}

}

%%  EDGES  %%
   \ncline{d}{s}
   \ncline{a}{Cl}
   \ncline{a}{d}
   \ncline{Cu}{s}

%%  MSGS  %%
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{<->}{Cl}{a}
   \aput[1pt]{:D}{\tiny \msg{RREQ}{s}{x}}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{<->}{s}{Cu}
   \aput[1pt]{:D}{\tiny \msg{RREQ}{s}{x}}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{<->}{a}{d}
   \aput[1pt]{:U}{\tiny \msg{RREQ}{s}{x}}
%   \ncline[linewidth=0.8pt,linecolor=blue,arrowsize=4pt,offset=2pt]{<-}{d}{a}
%   \aput[1pt]{:D}{\tiny \msg{RREQ}{s}{x}}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{<->}{d}{s}
   \aput[1pt]{:U}{\tiny \msg{RREQ}{s}{x}}
%   \ncline[linewidth=0.8pt,linecolor=blue,arrowsize=4pt,offset=2pt]{->}{s}{d}
%   \aput[1pt]{:D}{\tiny \msg{RREQ}{s}{x}}

\endpspicture


==> fig/ex_loop_5.tex <==
%% Latex Commands%%
\newcommand{\msg}[3]{#1${}_{\!\!\;\MakeUppercase{#2}\!\!\:\shortrightarrow\!\MakeUppercase{#3}}$}
\newcommand{\msgerr}{RERR}
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(5.0,2.0){0.28}{x}
   \rput(5.0,2.091){\small$X$}
   \rput(5.0,1.8599999999999999){\tiny $1$}
\rput(5.0,2.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}
   \rput(2.6,0.0){\includegraphics[scale=0.13]{cloud.eps}}
   \cnode(0.0,0.0){0.28}{a}
   \rput(0.0,0.091){\small$A$}
   \rput(0.0,-0.14){\tiny $1$}
\rput(0.0,-0.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (D & 2 & \mbox{val} & 1 & D)\\
       (S & 3 & \mbox{val} & 2 & D)\\
   \end{array}$}

}
   \pnode(2.5,0.45){Cu}
   \cnode(0.0,2.0){0.28}{d}
   \rput(0.0,2.091){\small$D$}
   \rput(0.0,1.8599999999999999){\tiny $2$}
\rput(0.0,2.71){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 1 & \mbox{val} & 1 & A)\\
       (D & 2 & \mbox{val} & 2 & A)\\
       (S & 3 & \mbox{val} & 1 & S)\\
   \end{array}$}

}
   \pnode(1.45,0.0){Cl}
   \cnode(2.5,2.0){0.28}{s}
   \rput(2.5,2.091){\small$S$}
   \rput(2.5,1.8599999999999999){\tiny $3$}
\rput(2.5,2.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (D & 2 & \mbox{val} & 3 & D)\\
   \end{array}$}

}

%%  EDGES  %%
   \ncline{d}{s}
   \ncline{a}{Cl}
   \ncline{a}{d}
   \ncline{Cu}{s}

%%  MSGS  %%
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{->}{Cl}{a}
   \aput[1pt]{:D}{\tiny \msg{RREQ}{s}{d}}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{->}{a}{d}
   \aput[1pt]{:U}{\tiny \msg{RREP}{s}{d}}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{->}{d}{s}
   \aput[1pt]{:U}{\tiny \msg{RREP}{s}{d}}

\endpspicture


==> fig/ex_loop_6.tex <==
%% Latex Commands%%
\newcommand{\msg}[3]{#1${}_{\!\!\;\MakeUppercase{#2}\!\!\:\shortrightarrow\!\MakeUppercase{#3}}$}
\newcommand{\msgerr}{RERR}
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(5.0,2.0){0.28}{x}
   \rput(5.0,2.091){\small$X$}
   \rput(5.0,1.8599999999999999){\tiny $1$}
\rput(5.0,2.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (D & 3 & \mbox{val} & 2 & S)\\
       (S & 0 & \mbox{val} & 1 & S)\\
   \end{array}$}

}
   \rput(2.6,0.0){\includegraphics[scale=0.13]{cloud.eps}}
   \cnode(0.0,0.0){0.28}{a}
   \rput(0.0,0.091){\small$A$}
   \rput(0.0,-0.14){\tiny $1$}
\rput(0.0,-0.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (D & 2 & \mbox{val} & 1 & D)\\
       (S & 3 & \mbox{val} & 2 & D)\\
   \end{array}$}

}
   \pnode(2.5,0.45){Cu}
   \cnode(0.0,2.0){0.28}{d}
   \rput(0.0,2.091){\small$D$}
   \rput(0.0,1.8599999999999999){\tiny $3$}
\rput(0.0,2.815){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 1 & \mbox{val} & 1 & A)\\
       (D & 2 & \mbox{val} & 2 & A)\\
       (S & 3 & \mbox{val} & 1 & S)\\
       (X & 1 & \mbox{val} & 2 & S)\\
   \end{array}$}

}
   \pnode(1.45,0.0){Cl}
   \cnode(2.5,2.0){0.28}{s}
   \rput(2.5,2.091){\small$S$}
   \rput(2.5,1.8599999999999999){\tiny $3$}
\rput(2.5,2.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (D & 3 & \mbox{val} & 1 & D)\\
       (X & 1 & \mbox{val} & 1 & X)\\
   \end{array}$}

}

%%  EDGES  %%
   \ncline{d}{s}
   \ncline{s}{x}
   \ncline{a}{Cl}
   \ncline{Cu}{s}

%%  MSGS  %%
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{<->}{s}{Cu}
   \aput[1pt]{:D}{\tiny \msg{RREQ}{d}{x}}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{->}{s}{d}
   \aput[1pt]{:D}{\tiny \msg{RREP}{d}{x}}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{->}{x}{s}
   \aput[1pt]{:D}{\tiny \msg{RREP}{d}{x}}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{<->}{d}{s}
   \aput[1pt]{:U}{\tiny \msg{RREQ}{d}{x}}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{->}{s}{x}
   \aput[1pt]{:U}{\tiny \msg{RREQ}{d}{x}}

\endpspicture


==> fig/ex_loop_7.tex <==
%% Latex Commands%%
\newcommand{\msg}[3]{#1${}_{\!\!\;\MakeUppercase{#2}\!\!\:\shortrightarrow\!\MakeUppercase{#3}}$}
\newcommand{\msgerr}{RERR}
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(5.0,2.0){0.28}{x}
   \rput(5.0,2.091){\small$X$}
   \rput(5.0,1.8599999999999999){\tiny $1$}
\rput(5.0,2.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (D & 3 & \mbox{val} & 2 & S)\\
       (S & 0 & \mbox{val} & 1 & S)\\
   \end{array}$}

}
   \rput(2.6,0.0){\includegraphics[scale=0.13]{cloud.eps}}
   \cnode(0.0,0.0){0.28}{a}
   \rput(0.0,0.091){\small$A$}
   \rput(0.0,-0.14){\tiny $1$}
\rput(0.0,-0.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (D & 2 & \mbox{val} & 1 & D)\\
       (S & 3 & \mbox{val} & 2 & D)\\
   \end{array}$}

}
   \pnode(2.5,0.45){Cu}
   \cnode(0.0,2.0){0.28}{d}
   \rput(0.0,2.091){\small$D$}
   \rput(0.0,1.8599999999999999){\tiny $3$}
\rput(0.0,2.815){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 2 & \mbox{inv} & 1 & A)\\
       (D & 3 & \mbox{inv} & 2 & A)\\
       (S & 3 & \mbox{val} & 1 & S)\\
       (X & 1 & \mbox{val} & 2 & S)\\
   \end{array}$}

}
   \pnode(1.45,0.0){Cl}
   \cnode(2.5,2.0){0.28}{s}
   \rput(2.5,2.091){\small$S$}
   \rput(2.5,1.8599999999999999){\tiny $3$}
\rput(2.5,2.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (D & 3 & \mbox{inv} & 1 & D)\\
       (X & 1 & \mbox{val} & 1 & X)\\
   \end{array}$}

}

%%  EDGES  %%
   \ncline{d}{s}
   \ncline{a}{Cl}
   \ncline{Cu}{s}

%%  MSGS  %%
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{->}{d}{s}
   \aput[1pt]{:U}{\tiny \msgerr}

\endpspicture


==> fig/ex_loop_8.tex <==
%% Latex Commands%%
\newcommand{\msg}[3]{#1${}_{\!\!\;\MakeUppercase{#2}\!\!\:\shortrightarrow\!\MakeUppercase{#3}}$}
\newcommand{\msgerr}{RERR}
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(5.0,2.0){0.28}{x}
   \rput(5.0,2.091){\small$X$}
   \rput(5.0,1.8599999999999999){\tiny $1$}
\rput(5.0,2.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (D & 3 & \mbox{val} & 2 & S)\\
       (S & 4 & \mbox{val} & 1 & S)\\
   \end{array}$}

}
   \rput(2.6,0.0){\includegraphics[scale=0.13]{cloud.eps}}
   \cnode(0.0,0.0){0.28}{a}
   \rput(0.0,0.091){\small$A$}
   \rput(0.0,-0.14){\tiny $1$}
\rput(0.0,-0.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (D & 2 & \mbox{val} & 1 & D)\\
       (S & 3 & \mbox{val} & 2 & D)\\
   \end{array}$}

}
   \pnode(2.5,0.45){Cu}
   \cnode(0.0,2.0){0.28}{d}
   \rput(0.0,2.091){\small$D$}
   \rput(0.0,1.8599999999999999){\tiny $3$}
\rput(0.0,2.815){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 2 & \mbox{inv} & 1 & A)\\
       (D & 3 & \mbox{inv} & 2 & A)\\
       (S & 3 & \mbox{val} & 1 & S)\\
       (X & 1 & \mbox{val} & 2 & S)\\
   \end{array}$}

}
   \pnode(1.45,0.0){Cl}
   \cnode(2.5,2.0){0.28}{s}
   \rput(2.5,2.091){\small$S$}
   \rput(2.5,1.8599999999999999){\tiny $4$}
\rput(2.5,2.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (D & 3 & \mbox{val} & 3 & X)\\
       (X & 1 & \mbox{val} & 1 & X)\\
   \end{array}$}

}

%%  EDGES  %%
   \ncline{s}{x}
   \ncline{a}{Cl}
   \ncline{Cu}{s}

%%  MSGS  %%
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{->}{x}{s}
   \aput[1pt]{:D}{\tiny \msg{RREP}{s}{d}}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{->}{s}{x}
   \aput[1pt]{:U}{\tiny \msg{RREQ}{s}{d}}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=2pt]{<->}{s}{Cu}
   \aput[1pt]{:D}{\tiny \msg{RREQ}{s}{d}}

\endpspicture


==> fig/good_loop_sketch.tex <==
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(-0.5,0){0.25}{a}
   \rput(-0.5,0){$A$}
   \cnode(0.5,0){0.25}{c}
   \rput(0.5,0){$C$}
   \cnode(0,0.866){0.25}{b}
   \rput(0,0.866){$B$}
   
   \cnode[linecolor=lightgray](1.366,-0.5){0.25}{d1}
   \rput(1.366,-0.5){\textcolor{lightgray}{$D$}}
   \cnode[linecolor=lightgray](-1.366,-0.5){0.25}{d2}
   \rput(-1.366,-0.5){\textcolor{lightgray}{$D$}}
   \cnode(0,1.866){0.25}{d3}
   \rput(0,1.866){$D$}

%%  EDGES  %%
   \ncline{a}{b}
   \ncline{b}{c}
   \ncline{c}{a}
   \ncline[linecolor=lightgray]{c}{d1}
   \ncline[linecolor=lightgray]{a}{d2}
   \ncline{b}{d3}
   
    \psarc[linecolor=lightgray,linestyle=dashed,linewidth=0.2pt,arrowsize=6pt]{<-}(0,0.288){1.578}{-21}{81}
    \psarc[linecolor=lightgray,linestyle=dashed,linewidth=0.2pt,arrowsize=6pt]{<-}(0,0.288){1.578}{219}{-39}
    \psarc[linecolor=lightgray,linestyle=dashed,linewidth=0.2pt,arrowsize=6pt]{<-}(0,0.288){1.578}{99}{201}

\endpspicture

